Evaluating and Enhancing Out-of-Domain Generalization of Task-Oriented Dialog Systems for Task Completion without Turn-level Dialog Annotations

Traditional task-oriented dialog (ToD) systems rely heavily on labor-intensive turn-level annotations, such as dialogue states and policy labels, for training. This work explores whether large language models (LLMs) can be fine-tuned solely on natural language dialogs to perform ToD tasks, without requiring such annotations. We evaluate their ability to generalize to unseen domains and compare their performance with models trained on fully annotated data. Through extensive experiments with three open-source LLMs of varying sizes and two diverse ToD datasets, we find that models fine-tuned without turn-level annotations generate coherent and contextually appropriate responses. However, their task completion performance - measured by accurate execution of API calls - remains suboptimal, with the best models achieving only around 53% success in unseen domains. To improve task completion, we propose ZeroToD, a framework that incorporates a schema augmentation mechanism to enhance API call accuracy and overall task completion rates, particularly in out-of-domain settings. We also compare ZeroToD with fine-tuning-free alternatives, such as prompting off-the-shelf LLMs, and find that our framework enables smaller, fine-tuned models that outperform large-scale proprietary LLMs in task completion. Additionally, a human study evaluating informativeness, fluency, and task completion confirms our empirical findings. These findings suggest the feasibility of developing cost-effective, scalable, and zero-shot generalizable ToD systems for real-world applications.

==> my_files/map.tex <==


Research questions
\begin{itemize}
\item Do we need turn level annotations No
\item Do llms generalize to unseen domain in TOD context Yes
\item Is prompting enough No
\item Do LLMs complete task No
\item with augmentation Yes
\item Is there any benefits of fine-tuning for generalization Yes

\end{itemize}

Introduction
\begin{itemize}
    \item Introduce TOD
    \item Manual Annotation
    \item Limitations of annotations
    \item API calls
    \item SOTA avoid API calls
    \item Pretrained LLMs do generalize
    \item Good in generic domains(alarm, services, weather, media), struggle in complex domains (hotels, ridesharing, trains, events, restaurants)
    \item Our proposals
    \item no annotations required, allows to use existing data
    \item make api calls
    \item Generalizes and handles complex domains
    \item Eval on 2 dataset, LLMs of different sizes, ablation study for augmentation
    \item Results better than SOTA models trained on annotated data and AUTO TOD.
\end{itemize}

Results
Focus more on API calls
Very little discussion on Response Generation
Show domain wise results of nltod with auto tod to show that auto tod struggles on certain domains and nltod is consistent across domains
Ablation study of augmentation, show example of party size and num of people 


Drop?
\begin{itemize}
    \item Mixed
    \item Detailed performance across NL-TOD model with different sizes
    \item Replace with abalation study of manual annotation
    \item Multi domain
\end{itemize}
